GREX-PLUS Science Book v2

GREX-PLUS (Galaxy Reionization EXplorer and PLanetary Universe Spectrometer) is a mission candidate for a JAXA strategic L-class mission to be launched in the 2030s. Its primary science goals are two-fold: galaxy formation and evolution, and planetary system formation and evolution. The GREX-PLUS spacecraft will carry a telescope with a 1 m primary mirror aperture cooled down to 50 K. The two science instruments will be onboard: a wide-field camera in the 2--8 $\mu$m wavelength band and a high-resolution spectrometer with a wavelength resolution of 30,000 in the 10--18 $\mu$m band. The GREX-PLUS wide-field camera aims to detect the first generation of galaxies at redshift $z>15$. The GREX-PLUS high-resolution spectrometer aims to identify the location of the water ``snowline'' in protoplanetary disks. Both instruments will provide unique datasets for a broad range of scientific topics, including galaxy mass assembly, the origin of supermassive blackholes, infrared background radiation, molecular spectroscopy in the interstellar medium, transit spectroscopy of exoplanet atmospheres, planetary atmospheres in the Solar System, and so on. This document is the second version of a collection of scientific themes that can be achieved with GREX-PLUS. Each section in Chapters~2 and 3 is based on presentations at several GREX-PLUS Science Workshops.

==> 2-3_lssandmassassembly/lssandmassassembly_v1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Science Cases
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% For biblatex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{refsection}[2-3_lssandmassassembly/lssandmassassembly.bib]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Large Scale Structure and Galaxy Mass Assembly History}
\label{sec:lssandmassassembly}

%--- Authors ---------------------------------------------------
\noindent
\begin{flushright}
%% Authors
Tadayuki Kodama$^{1}$, 
Yusei Koyama$^{2}$,
Ken Mawatari$^{2}$
\\
$^{1}$ Tohoku University, 
$^{2}$ NAOJ 
\end{flushright}
\vspace{0.5cm}
%---------------------------------------------------------------


\subsection{Scientific background and motivation}

In the contemporary standard universe which is dominated by cold dark matter, smaller scale density fluctuations tend to have larger amplitudes in the early universe. Therefore, small low-mass objects are born first in the early universe and more massive objects are grown later by the gravitational assembly and mergers of smaller objects.
To reveal the mass assembly history of galaxies and clusters of galaxies is the fundamental approach to understand the formation and evolution of these objects, and to test the above standard theory of the universe.
If the unexpectedly large, massive galaxies are discovered in the early universe, they would force us to modify our standard views of the universe and the nature of dark matter.

In order to trace the galactic scale mass assembly history, we must observe all the way from the early building blocks of galaxies with stellar masses of 10$^9$ M$_{\odot}$ (equivalent of $\sim$ 1 per cent
of our present-day Milky Way galaxy) to the most massive galaxies with 10$^{12}$ M$_{\odot}$ (10 times larger than the MW) and sketch how the mass are grown across the cosmic times.
Mass assembly consists of two processes, star formation within individual galaxies and mergers with other galaxies. During mergers, some involve intense new star formation while others do not and just add the existing stellar masses.
These processes and their timescales are also known to depend on the surrounding environments (host halo masses and the number density of nearby galaxies), which must be closely related to the strong environmental dependence of galaxy properties (such as morphology and star formation activity) in the present-day universe.

Therefore, we aim to construct stellar mass functions (SMF) covering the full stellar mass range from the building blocks to most massive galaxies, and compare the SMF as a function of cosmic time (all the way from the early epoch to the present-day) and environment (from dense cluster cores to the general field) in detail, which will enable us to obtain the complete picture of galaxy mass assembly.

We will search for ultra massive galaxies at $z>4$ taking the advantage of our large survey volume. Existence of such massive galaxies in the early universe will put strong constraints on the hierarchical galaxy formation theory in the context of cold dark-matter dominated universe, because there is little time available for such massive galaxies to grow in the early universe. Such surveys have already been done to $z\sim4$ with ground-based NIR observations \citep{2018A&A...618A..85S}.
The higher-$z$ entention to $z\sim5$ of the survey is currently undergoing with medium-band filters at the K-band (K1,K2,K3 and K4) on SWIMS and MOIRCS which can capture Balmer-break features to $z\sim5$ (Ruby-Rush project; Kodama et al.).
We now want to extend the survey further back in time with GREX-PLUS utilizing its longer wavelength coverage and the wide field of view.

For these purposes, it is essential for us to observe distant galaxies at the rest-frame optical wavelength ($>$0.5 nm). So far, we have been largely limited to $z$=4 by ground-based observations up to 2$\mu$m (K-band). Above that wavelength (and  that redshift), ground-based observations would severely suffer from high background noise. Moreover, massive galaxies are rare on the sky and thus large area surveys are required. Space observations with GREX-PLUS is extremely unique and can play absolute key roles here because of its longer wide wavelength coverage (up to 8 $\mu$m), and its wide field of view (0.25 degree$^2$).

Moreover, we aim to conduct the clustering analyses of galaxies (and clusters as well) by utilizing the contiguous, extremely large survey data that GREX-PLUS can provide.
The clustering strength of galaxies that we can measure is a good proxy of underlying dark matter halo mass which host those galaxies. Thus we can derive stellar to halo mass ratio (SHMR) back to $z\sim8$ or so, which is also a key physical quantity that describes the galaxy formation efficiency and thus gives us crucial insights into the formation and evolution of galaxies.
In order to also investigate galaxy cluster/group scale haloes and their surrounding large scale structures, we need to cover at least 100 Mpc in comoving scale. For a statistical analysis, we request a survey over a 10 square degree area.

The most accurate stellar mass measurements can be done at the rest-frame near-infrared (NIR) wavelength (1.6--2 $\mu$m), because the mass-to-light ratio is relatively constant over various stellar populations and its scatter is at least several times smaller than the other bands.
For example, we can obtain precise stellar masses of Lyman break galaxies (LBGs) or typical star forming galaxies at $z\sim3$.
We can also calibrate the previous stellar masses measured based on rest-frame optical light with our more accurate stellar masses to be obtained.  We can thus improve the conversion equation to derive stellar masses for various galaxies with various star formation histories,

\subsection{Required observations and expected results}

Figure~\ref{fig:masslim} shows the limiting stellar mass as a function of redshift that can be detected at 5$\sigma$ with GREX-PLUS.
In order to detect building blocks of galaxies with 10$^9$ M$_{\odot}$/yr back to $z\sim8$, we must reach down to 27 AB magnitudes, well matched to our planned observations.
By combining with Subaru/HSC optical imaging data, we can cover the wavelength range of 0.4--5 (and up to 8 for bright galaxies) $\mu$m, and thus can measure stellar masses precisely from the spectral energy distribution (SED) of galaxies.

We can also conduct a statistical number count of close neighbour galaxies utilizing the relatively high spatial resolution of GREX-PLUS in order to investigate the relative contribution of galaxy mergers to the mass assembly history.
The required spatial resolution for this purpose is 8 kpc or 1 arcsec so that we can resolve neighbouring galaxies beyond the cosmic noon epoch ($z>2$).

We aim to construct a large statistical sample of galaxies across the cosmic age and environment with a large area survey. We also need to map the growth history of large scale structures back to $z\sim8$.
The 100 square-degree is a sufficiently large area that corresponds to the comoving volume which can include the progenitors of 100 present-day rich galaxy clusters like Coma. This will enable us to conduct the statistical and quantitative analyses.

We can separate the two major processes of mass assembly, namely star formation and mergers, and thus can track the mass assembly history of galaxies all the way from the building blocks in the early universe to the mature galaxies in the present-day universe. We will also investigate its dependence on galaxy morphology and surrounding environment.
%%
We will also trace the mass assembly history of large scale structures by observing the full range of environments, from rich cluster cores to the surrounding large filamentary structures.

For the precise stellar mass measurements based on rest-frame NIR light, we aim to observe LBGs at $z\sim3$ at 5--8 $\mu$m.
The typical stellar mass of LBGs based on the rest-frame optical light is around 10$^{10-11}$ M$_{\odot}$ (e.g., \citealt{2010MNRAS.401.1521M}), which corresponds to 25--24 AB magnitudes in the rest-frame NIR, if the mass-to-light ratio calibrated at the nearby universe is used \citep{2003ApJS..149..289B}.
A 10 square-degree survey can construct a sample of more than several 1000 LBGs, statistically sufficient for the above analysis.

\subsection{Scientific goals}

\begin{itemize}
\item Detect building blocks of galaxies down to 10$^9$ M$_{\odot}$ back to $z\sim8$, and construct stellar mass functions.
\item Find massive galaxies at $z>4$, and put constraints on the hierarchical galaxy formation theories.
\item Find 100 progenitors within each $\Delta$$z$=1 slice,
and trace the mass assembly history of galaxy clusters and large scale structures.
\item Observe 1000 LBGs at $z\sim3$ and measure precise stellar masses based on rest-frame NIR light, and calibrate the conventional stellar mass measurement method based on the rest-frame optical light.
\end{itemize}

\begin{figure}
    \begin{center}
      \includegraphics[width=8cm]{2-3_lssandmassassembly/masslim.png}
    \end{center}
    \caption{Limiting stellar mass of galaxies as a function of redshift with GREX-PLUS. If we reach 26--27 AB magnitudes at F232 (2.3$\mu$m), F303 (3.0$\mu$m), and F397 (4.0$\mu$m) as specified in the figure, we will be able to trace the stellar mass assembly history back to $z\sim8$ and down to the building blocks of 10$^9$ M$_{\odot}$ or 1/100 of our Milky Way galaxy.}\label{fig:masslim}
\end{figure}

\begin{table}[ht]
    \label{tab:lssandmass}
    \begin{center}
    \caption{Required observational parameters.}
    \begin{tabular}{|l|p{9cm}|l|}
    \hline
     & Requirement & Remarks \\
    \hline
    Wavelength & 2--8 $\mu$m & \multirow{2}{*}{$a$} \\
    \cline{1-2}
    Spatial resolution & $<1$ arcsec & \\
    \hline
    Wavelength resolution & $\lambda/\Delta \lambda>3$ & $b$ \\
    \hline
    Field of view & 2--5 $\mu$m: 10 degree$^2$, 27 ABmag ($5\sigma$, point-source) & \multirow{2}{*}{$c$}\\
    \cline{1-1}
    Sensitivity & 5--8 $\mu$m 10 degree$^2$, 24--25 ABmag ($5\sigma$, point-source) & \\
    \hline
    Observing field & Fields where deep imaging data at $\lambda<2$ $\mu$m are available. & $d$ \\
    \hline
    Observing cadence & N/A & \\
    \hline
    \end{tabular}
    \end{center}
    $^a$ Primary mirror $\phi>1.2$ m is required to achieve $<1$ arcsec at $\lambda=5$ $\mu$m for the diffraction limit.\\
    $^b$ Three or more bands are required for the color selection of very high-$z$ galaxies.\\
    $^c$ A $>0.25$ degree$^2$ field-of-view of a single pointing is required from the point-source sensitivity for a $\phi=1.2$ m telescope and a supposed amount of observing time.\\
    $^d$ For example, deep fields observed with Subaru and Roman.
\end{table}

% References
\printbibliography[heading=subbibliography]
\end{refsection}


